GiPH: Generalizable Placement Learning for Adaptive Heterogeneous Computing

Careful placement of a computational application within a target device cluster is critical for achieving low application completion time. The problem is challenging due to its NP-hardness and combinatorial nature. In recent years, learning-based approaches have been proposed to learn a placement policy that can be applied to unseen applications, motivated by the problem of placing a neural network across cloud servers. These approaches, however, generally assume the device cluster is fixed, which is not the case in mobile or edge computing settings, where heterogeneous devices move in and out of range for a particular application. We propose a new learning approach called GiPH, which learns policies that generalize to dynamic device clusters via 1) a novel graph representation gpNet that efficiently encodes the information needed for choosing a good placement, and 2) a scalable graph neural network (GNN) that learns a summary of the gpNet information. GiPH turns the placement problem into that of finding a sequence of placement improvements, learning a policy for selecting this sequence that scales to problems of arbitrary size. We evaluate GiPH with a wide range of task graphs and device clusters and show that our learned policy rapidly find good placements for new problem instances. GiPH finds placements with up to 30.5% lower completion times, searching up to 3X faster than other search-based placement policies.

==> 3_framework.tex <==

\section{GiPH}
\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{figs/p2.pdf}
    \caption{MDP (Markov decision process) of the placement search for a 2-task graph on 3 devices.}
    \label{fig:p2}
\end{figure}
This section introduces GiPH. Each subsection describes the key ideas: the formulation of the search problem and the associated Markov decision process (MDP) that enable an RL formulation (\cref{sec:mdp}), a novel gpNet representation of the information needed to find a placement (\cref{sec:representation}), a scalable neural network design to summarize gpNet's graph representation (\cref{sec:design}), and RL training to learn a good placement search policy (\cref{sec:train}).

\subsection{Markov Decision Process Formalism}\label{sec:mdp}

We formulate the placement problem as a search problem, where given an initial placement, {a learned policy} iteratively applies some small changes to the current placement. Through making these incremental changes\edited{, i.e., task relocation}, the policy is able to search through the solution space and find better placement solutions. Instead of trying to learn a policy that places the whole graph at once,  our search approach makes the learning simpler by only considering a small local search space at a time. {Focusing on incremental changes further allows us to generalize to arbitrary application task graphs and device clusters (\cref{sec:design}).} 

\paragraph{State} Consider a single problem instance  $(G,N)$. For the search problem, we define the \textit{state space} as the set of all feasible placements $S_{G,N}=\{\mathcal{M}|\mathcal{M}(v_i)\in D_i,\forall v_i\in V\}$. (\textit{State} and \textit{placement} terms are  interchangeably used in the paper.) The size of the state space $|S_{G,N}|=\prod_{i=0}^{|V|-1} |D_i|$, since each task can be placed on any of the feasible devices for it. When there is no placement constraint { (i.e., $D_i=D$ for all tasks)}, $|S_{G,N}|=|D|^{|V|}$. For the two-task example shown in Fig.~\ref{fig:p2}(a), there are a total of 4 feasible placements, all shown as states in the transition diagram of Fig.~\ref{fig:p2}(b). 

\paragraph{Action} To search through the state space, we define an \textit{action} to be a task and device pair $(v_i, d_j)\in V\times D$ that sets the placement of $v_i$ to device $d_j$. {Unlike Placeto~\citep{addanki2019placeto} that visits each task exactly once,  our search policy also decides the next task to visit given the current placement. By including task selection in action, we allow the policy to relocate tasks in any order and for more than once. In this way, the search-based policy can go back and adjust the placement of the same task again after moving others tasks, exploring the state space. Placeto traverses the nodes in an arbitrary order, which impedes its ability to fully explore possible placement options. } %Suppose at time $t$, the current state $s_t=\mathcal{M}$. If $\mathcal{M}(v_i)=d_j$, the action does not change the current placement and $s_{t+1}=s_t=\mathcal{M}$. If $\mathcal{M}(v_i)\neq d_j$, the action moves the  placement of $v_i$ from $\mathcal{M}(v_i)$ to $d_j$,  and $s_{t+1}=\mathcal{M}'\neq\mathcal{M}$ such that $\mathcal{M}'(v_i)=d_j$ and $\mathcal{M}'(v_k)=\mathcal{M}(v_k)$ for all $k\in [n]/i$. 

We only consider feasible actions $(v_i,d_j)$ such that $d_j\in D_i$. The size of the action space is thus $|A_{G,N}|=\sum_{i=0}^{|V|-1}|D_i|$, which is $|V||D|$ if there are no placement constraints. Fig. \ref{fig:p2}(b) lists all four actions for the simple two-task example and shows the deterministic state transition given an action taken at each state.
%
Note that the diameter, i.e., the length of the longest shortest path between any two states in the state transition diagram, is $|V|$ because one can always change from one placement to any other placement by moving each task node at most once. Therefore, even though the state space grows exponentially with $|V|$, we can reach any state from any other state in $|V|$ steps. 

\paragraph{Reward} The \textit{objective function} $\rho(\mathcal{M}|G,N)$ reflects how good a state $s=\mathcal{M}$ is. We assign intermediate reward  $r_t= \rho(s_{t+1}|G,N)-\rho(s_{t}|G,N)$, which mimics the advantage function \cite{rl} indicating the performance improvement after taking an action $a_t$ at a given state $s_t$. The goal of RL is to learn to take actions in order to maximize the  expected return $\sum_{t=0}^{T}\gamma^tr_t$, where $T$ is the  episode length. When $\gamma=1$, the expected return is the expected performance improvement between the final state $s_{T}$ and a randomly initialized state $s_0$, i.e., the policy tries to maximize $\mathbb{E}[\rho(s_{T}|G,N)] - \mathbb{E}[\rho(s_{0}|G,N)]$. Since the latter term is constant for a $(G,N)$ pair  with random initialization, RL is effectively improving the expected performance of the final placement through maximizing the expected return. When $\gamma < 1$, the policy seeks more immediate reward as future rewards are discounted. In this case, the policy also learns to search more efficiently {(i.e., increase the reward the most)} at the beginning of the RL episodes.   

We consider the MDP (Markov Decision Process) for the placement of a task graph $G$ on a device network $D$ as follows. At first, we initialize a random placement $s_{0}\sim |S_{G,N}|$, where each task node is randomly assigned to one of the feasible devices.  At each step $t$, an action $a_t\in A_{G,N}$ is taken to update the current placement $s_t$ and transition to the next state $s_{t+1}$. {A reward $r_t$ indicating the performance improvement after taking the action is received. An episode ends when the performance does not change significantly over multiple steps. }

% mention placeto and compare


\subsection{gpNet Representation}\label{sec:representation}
We have formulated a discrete MDP for the placement search problem given $(G,N)$.  However, for the learned policy to be fully generalizable without depending on $(G,N)$, a representation of a general placement $\mathcal{P}=(G,N,\mathcal{M}^{G\rightarrow N})$ is required to work across different problem instances with an arbitrary pair of task graph and device network. The representation should capture the heterogeneous compute and communication requirements of the task graph $G$ and the heterogeneous compute and communication capabilities of the device network $N$, in order to learn the relation between $\rho$ and $\mathcal{P}$.

%The performance objective $\rho$ is likely to highly depend on those graph and network features. In order to enable the learning of the relation between $\rho$ and $\mathcal{P}$ and generalize across different task graphs and device networks, a flexible and general way of representing the placement with features and constraints is required. 

To this end, we present \textbf{gpNet}, a novel and universal graph representation of the placement that encapsulates features of both the task graphs and the device networks with placement constraints. gpNet generates a unique graph $H=(V_H,E_H)$ given a general placement $\mathcal{P}=(G,N,\mathcal{M}^{G\rightarrow N})$, where $G=(V,E)$ is an arbitrary task graph with node features $\bm{\beta}^n$ and edge features $\bm{\beta}^e$, and $N$ is an arbitrary device network composed of a device cluster $D$ with device compute features $\bm{b}^n$ and communication link features $\bm{b}^e$. $H\leftarrow gpNet\left(G=(V,E,\bm{\beta}^n,\bm{\beta}^e),N=(D,\bm{b}^n,\bm{b}^e),\mathcal{M}^{G\rightarrow N}\right)$.


\paragraph{Node generation} $V_H=\{(v_i,d_j)| d_j\in D_i \textrm{ for } i=0,...,|V|-1\}$. Each node in $H$ represents a feasible placement of $v_i\in V$ on device $d_j\in D_i$, and is labeled $(v_i,d_j)$, e.g., Fig.~\ref{fig:p1}(c)%\carlee{In general, put a space between Fig. and the figure number}
. The node feature $x^n_u$ of a node $u=(v_i,d_j)$ is a function, $f_n$, of the task feature $\beta^n_i$ and the device feature $b^n_j$, i.e., $x^n_u=f_n(\beta^n_i, b^n_j)$. The set of nodes for all possible placements of a task $v_i$ forms a group of placement options  $O_i=\{(v_i,\cdot) \}\subseteq V_H$. Nodes whose labels are in the current placement $\mathcal{M}^{G\rightarrow N}$ are called \textit{pivots} and form a set $V_{H,\mathcal{P}}\subseteq V_H$. The subgraph induced by $V_{H,\mathcal{P}}$ thus contains all information about the current placement $\mathcal{M}^{G\rightarrow N}$. Non-pivot nodes, on the other hand, represent a potential task \emph{re-placement}.  Each node in $H$ also corresponds to one action defined in the search problem described in \cref{sec:mdp}. This correspondence is exploited later in our neural network design (\cref{sec:design}).  

\paragraph{Edge generation} We add edge $(u_1,u_2)$ with $u_1=(v_i,d_k), u_2=(v_j,d_l)$ to the gpNet  $H$ if $(v_i,v_j)\in E$ and at least one of $u_1$ and $u_2$ is a pivot, i.e., $u_1\in V_{H,\mathcal{P}}\textrm{ or }u_2\in V_{H,\mathcal{P}}$.  In this way,  each non-pivot  node $(v_i,d_j)$  only has edges pointing to or from pivots that contain the current placement information of its parent and child tasks. For example, in Fig.~\ref{fig:p1}(c), $(v_1,d_2)$ has an incoming edge from $(v_0,d_0)$, which contains the {current} placement information of $v_1$'s parent task $v_0$,  and outgoing edges to $(v_3,d_2)$ and $(v_4,d_1)$, which contain the {current} placement information of $v_1$'s child tasks $v_3$ and $v_4$.  Thus,  \emph{non-pivot node $(v_i,d_j)$ has a local graph structure corresponding to $v_i$ being re-placed to $d_j$}. The edge feature $x^e_{u_1u_2}$ of $(u_1=(v_i,d_k), u_2=(v_j,d_l))$  is a function, $f_e$, of the data link features $\beta^e_{ij}$ and the communication link features $b^e_{kl}$.%, i.e., $x^e_{u_1u_2}=f_e(\beta^e_{ij}, b^e_{kl})$. 
The resulting graph $H$ has $|V_H|=\sum_{i=0}^{|V|-1}|D_i|$ nodes and $|E_H|=\sum_{i=0}^{|V|-1}\left(|D_i||E_i|\right) - |E|$ edges, where $|E_i|$ is the degree of $v_i$ in $G$. Both $f_n$ and $f_e$ can be any functions that combine the features of the task graph and the device network (e.g., concatenation).


{See Appendix \ref{alg:gpnet} for the full algorithm.} Our proposed gpNet unifies a given application graph $G$ and device cluster $N$ into a single graph that \emph{captures all device- and task-related features} for making a placement update decision. The original task dependencies in $G$ and placement constraints are implicitly present in the output gpNet $H$ by construction.  gpNet also generalizes to different problem instances: we can construct a gpNet for any placement of an arbitrary task graph-device network problem pair $(G,N)$.%, and it unifies the application graph and device network into a single graph with all relevant features for finding good placements. 


\subsection{Neural Network Design}\label{sec:design}
\begin{figure*}
    \centering
    \includegraphics[width=.9\linewidth]{figs/p3.pdf}
    \caption{GiPH neural network design. A given problem instance $(G_i, N_i)$ is first transformed into a graphical gpNet representation, which is then passed through a GNN to generate feature embeddings for each feasible task-device placement pair. The policy network then chooses an action (an incremental task-device re-placement) by estimating its performance improvement.}
    \label{fig:p3}
\end{figure*}

The learning framework of GiPH is shown in Fig. \ref{fig:p3}. Given a placement problem of an arbitrary task graph $G_i$ and target network $N_i$, the placement agent starts a search  from a randomly initialized placement $\mathcal{M}^{G_i\rightarrow N_i}_0$. The agent then takes as the input the current state of the search, $\mathcal{P}=(G_i,N_i,\mathcal{M}^{G_i\rightarrow N_i}_t)$, decides a placement update (an action, as defined in \cref{sec:mdp}) that modifies the current placement, and observes the improvement of the objective $\rho$ as the reward. It includes a graph neural network and a policy network, which are jointly trained. Since we may have input gpNets of arbitrary sizes, instead of using a fixed-size policy network, the GiPH policy network  adopts a score function to evaluate individual actions {(i.e., nodes in gpNet), based in their local graph connectivity and encoded placement information}. Thus, it \emph{does not depend on the size of gpNet}. 

\paragraph{Scalable and generalizable graph embedding}
 GiPH must first convert the placement information, represented in graphical form by $gpNet(G_i,N_i,\mathcal{M}^{G_i\rightarrow N_i}_t)$, into features that can be passed to the policy network. 
 %gpNet (\cref{sec:representation})  generates a graph representation $gpNet(G_i,N_i,\mathcal{M}^{G_i\rightarrow N_i}_t)$ of the current state, but we still need to encode the graph-structured  information. 
 Creating a flat vector representation is not scalable because it cannot handle graphs of arbitrary sizes and shapes (which depend on the specific task graph, target network and constraints). 
 
 GiPH achieves scalability using a graph neural network (GNN)\citep{learn_graph,Battaglia2018RelationalIB} that embeds the state information in a set of embedding vectors. Taking a gpNet as input with node features $\bm{x}^n$ and edge features $\bm{x}^e$ composed as described in \cref{sec:representation}, GiPH propagates information in a sequence of message passing:
 \begin{equation}\label{eq:embedding}
     e_u=h_2\left(\sum_{v\in \xi(u)}h_1\left([e_v\mathbin\Vert x_{vu}^e]\right)\right) + x_u^n,
 \end{equation}
 for each node $u$ in the gpNet, where $\xi(u)$ is the set of parents of $u$, who have aggregated messages from all of their parents. $h_1(\cdot)$ and $h_2(\cdot)$  are non-linear transformations over vector inputs with trainable parameters. The message passing is done in both forward and backward directions  with separate parameters, each summarizing information about the subgraph of nodes that can be reached %and is reachable from \carlee{``can be reached'' is the same as ``is reachable from''. Do you mean the nodes 
 {from  $u$ and nodes that can reach $u$}.
GiPH concatenates the two summaries along each direction as the embedding of a node in gpNet. For a node with label $(v,d)$, this embedding thus captures the local placement information if $v$ is placed on $d$ (i.e., if an action $(v,d)$ is taken). %\carlee{This point may be worth elaborating on--remind the reader that the neighbors of a node in gpNet are exactly alternative placements.}
 %
 Adopting a GNN also helps generalizability because it automatically learns high-level features that are statistically important through end-to-end training, and the model learned can generalize (and scale) to unseen graphs.
 

\paragraph{Policy network and actions} The policy network consists of a multi-layer perceptron (MLP), an optional mask layer, and a softmax layer (Fig. \ref{fig:p3}). We use the per-node embedding from the GNN to compute a score $q_a=g(e_a)$ for each action $a$ in the action space $ A_{G_i,N_i}$ (represented as nodes in the gpNet). $g(\cdot)$ is a score function implemented as a MLP that computes a scalar value for an embedding vector. The score $q_a$ quantifies how good an action is given the current state $s$. GiPH then uses a softmax layer to output a probability of selecting each action based on the score $P(a|s)={\exp{(q_a)}}/{\sum_{b\in A_{G_i,N_i}}\exp{(q_b)}}$. An optional mask layer can be placed before the softmax  to mask out undesired actions. The final output is a probability distribution over all feasible actions.

\subsection{RL Training}\label{sec:train}
GiPH uses a policy gradient method REINFORCE for training~\citep{reinforce}. During each episode, a placement problem $(G, N)$ is sampled from a training set $\mathcal{G}_T\times \mathcal{N}_T$. Starting from a random placement $s_0$, the agent collects observations $(s_t,a_t,r_t)$ at each step $t=0,...,T$ following the current policy $\pi_\theta$. It updates its policy parameters at the end of each episode
\begin{equation*}\label{eq:reinforce}
    \theta\leftarrow \theta + \alpha \sum_{t=0}^{T}\gamma^t\nabla_\theta\log \pi_\theta (a_t|s_t)\left(\sum_{t'=t}^{T}\gamma^{t'-t}r_{t'}-b_{t}\right),
\end{equation*}
where $\alpha$ is the learning rate, $\gamma$ is the discounting factor, and $b_t$ is a baseline for reducing the variance of the policy gradient~\citep{rl_baseline}. %It \carlee{does ``it'' mean 
{$b_t$} can be any function as long as it does not depend on the action {at time $t$}. We set it to be the average reward before step $t$ in an episode. 

 To improve the sample efficiency and force exploration, we mask out actions that do not change the current placement (e.g., $a_0,a_1$ at state $\mathcal{M}_0$ in the example Fig. \ref{fig:p2}(b)) because no new information will be acquired by taking those actions. We also mask out actions that will result in moving the same task consecutively twice because the latter action makes the former a redundant move. 
